Constraining Primordial Black Holes using Fast Radio Burst Gravitational-Lens Interferometry with CHIME/FRB

Fast radio bursts (FRBs) represent an exciting frontier in the study of gravitational lensing, due to their brightness, extragalactic nature, and the compact, coherent characteristics of their emission. In a companion work [Kader, Leung+2022], we use a novel interferometric method to search for gravitationally lensed FRBs in the time domain using bursts detected by CHIME/FRB. There, we dechannelize and autocorrelate electric field data at a time resolution of 1.25 ns. This enables a search for FRBs whose emission is coherently deflected by gravitational lensing around a foreground compact object such as a primordial black hole (PBH). Here, we use our non-detection of lensed FRBs to place novel constraints on the PBH abundance outside the Local Group. We use a novel two-screen model to take into account decoherence from scattering screens in our constraints. Our constraints are subject to a single astrophysical model parameter -- the effective distance between an FRB source and the scattering screen, for which we adopt a fiducial distance of 1 parsec. We find that coherent FRB lensing is a sensitive probe of sub-solar mass compact objects. Having observed no lenses in $172$ bursts from $114$ independent sightlines through the cosmic web, we constrain the fraction of dark matter made of compact objects, such as PBHs, to be $f \lesssim 0.8$, if their masses are $\sim 10^{-3} M_{\odot}$.

==> burst_table_rows_only.tex <==
 FRB20190110C &  222.08 &  36 & 0.28   \\ % 25677682
 FRB20190117A &  393.22 &  48 & 2.22   \\ % 27052203
 FRB20190122C &  689.97 &  30 & \ensuremath{<} 0.1  \\ % 27687783
 FRB20190202B &  464.88 &  70 & 0.08   \\ % 29204654
 FRB20190224D &  752.89 &  55 & 0.01   \\ % 31644043
 FRB20190301A &  459.79 &  82 & 2.08   \\ % 32158184
 FRB20190303B &  193.50 &  47 & 1.61   \\ % 32328347
 FRB20190320B &  489.51 &  38 & 0.08   \\ % 33769804
 FRB20190417C &  320.28 & 123 & 0.57   \\ % 37129627
 FRB20190423D &  496.68 &  67 & 5.16   \\ % 37696333
 FRB20190430C &  400.41 & 102 & 0.04   \\ % 38440671
 FRB20190606A &  552.65 &  32 & 1.60   \\ % 40949542
 FRB20190609A &  316.71 &  58 & 12.13  \\ % 41208961
 FRB20190609C &  479.87 & 113 & 0.31   \\ % 41252817
 FRB20190621A &  195.49 &  39 & 3.56   \\ % 41866365
 FRB20190624B &  213.95 &  70 & 0.18   \\ % 42295086
 FRB20190625E &  188.51 &  93 & 1.81   \\ % 42435604
 FRB20190628B &  408.03 &  47 & 0.68   \\ % 42809769
 FRB20190708A &  849.34 &  45 & 0.38   \\ % 43354078
 FRB20190712A &  682.40 &  52 & 0.13   \\ % 43822123
 FRB20190715B &  182.29 &  35 & 0.04   \\ % 44290216
 FRB20190722B &  508.47 &  56 & 0.12   \\ % 45371331
 FRB20190804B &  716.07 &  37 & 7.11   \\ % 46643744
 FRB20191018A &  301.34 &  49 & 1.24   \\ % 58983056
 FRB20191020D &  222.14 &  29 & 7.20   \\ % 59240332
 FRB20191024B &  400.28 & 102 & 0.07   \\ % 59560503
 FRB20191025D &  249.13 &  84 & \ensuremath{<} 0.1  \\ % 59794378
 FRB20191029A &  188.80 &  92 & 1.48   \\ % 59993356
 FRB20191104D &  192.16 &  56 & 5.03   \\ % 60569049
 FRB20191106C &  330.70 &  25 & 20.59  \\ % 60792403
 FRB20191107C &  222.24 &  37 & 0.48   \\ % 60955229
 FRB20191113C &  617.81 &  44 & 2.43   \\ % 61706633
 FRB20191114A &  552.93 &  99 & 10.83  \\ % 61913156
 FRB20191116A &  221.80 &  29 & 1.16   \\ % 62352548
 FRB20191215A &  222.12 &  29 & 0.06   \\ % 65049940
 FRB20191219A &  349.02 & 199 & 6.58   \\ % 65511496
 FRB20191219F &  464.56 &  49 & 0.11   \\ % 65547659
 FRB20191223A &  393.07 &  47 & 8.33   \\ % 65982134
 FRB20191223C &  604.76 &  80 & 0.01   \\ % 66073531
 FRB20191225A &  683.91 &  49 & 0.71   \\ % 66294123
 FRB20191231A &  222.42 &  30 & 3.57   \\ % 66995325
 FRB20200104E &  349.83 & 195 & \ensuremath{<} 0.1  \\ % 67522832
 FRB20200109B &  745.48 &  55 & 1.05   \\ % 68252213
 FRB20200112A &  221.16 &  29 & 1.85   \\ % 68602622
 FRB20200112D &  863.44 &  45 & 0.79   \\ % 68600370
 FRB20200118D &  625.34 &  77 & 1.33   \\ % 69246471
 FRB20200120E &   87.84 &  42 & 0.45   \\ % 69541452
 FRB20200120H &  349.80 & 200 & 1.06   \\ % 69509443
 FRB20200122A &  103.54 &  41 & \ensuremath{<} 0.1  \\ % 69841193
 FRB20200122D &  103.56 &  41 & 1.29   \\ % 69975256
 FRB20200122E &  103.56 &  41 & \ensuremath{<} 0.1  \\ % 69975309
 FRB20200122J &  103.49 &  41 & 0.16   \\ % 69848452
 FRB20200124A &  580.11 &  72 & \ensuremath{<} 0.1  \\ % 70375108
 FRB20200127B &  351.34 &  57 & 0.23   \\ % 70836867
 FRB20200128A &  439.61 &  45 & 0.25   \\ % 71042240
 FRB20200203A &  349.74 & 199 & 3.37   \\ % 71665813
 FRB20200204B &  349.30 & 200 & \ensuremath{<} 0.1  \\ % 71784400
 FRB20200204D &  350.19 & 199 & 2.79   \\ % 71784833
 FRB20200204J &  348.89 & 193 & \ensuremath{<} 0.1  \\ % 71785167
 FRB20200204K &  411.17 &  47 & 14.05  \\ % 71834323
 FRB20200207A &  506.85 &  67 & 1.08   \\ % 72197704
 FRB20200212A &  174.18 &  67 & 0.04   \\ % 72662238
 FRB20200219B &  351.27 &  54 & \ensuremath{<} 0.1  \\ % 73676317
 FRB20200220G &  313.38 &  58 & \ensuremath{<} 0.1  \\ % 73804471
 FRB20200501A &  469.51 &  51 & 6.56   \\ % 82758778
 FRB20200502A &  412.10 &  47 & 1.78   \\ % 82793120
 FRB20200503B &  674.19 &  51 & 7.12   \\ % 82874344
 FRB20200505B &  760.81 &  37 & 0.34   \\ % 83036587
 FRB20200507A &  166.92 &  51 & 0.44   \\ % 83390274
 FRB20200510A &  290.92 &  40 & 0.09   \\ % 83744922
 FRB20200512A &  349.63 & 104 & 7.17   \\ % 83984528
 FRB20200513A &  349.20 & 104 & 1.64   \\ % 84081108
 FRB20200513B &  579.72 &  72 & 3.12   \\ % 84032182
 FRB20200515A &  523.26 &  43 & 14.48  \\ % 84271986
 FRB20200520B &  351.41 &  54 & 0.19   \\ % 84633456
 FRB20200525A &  471.35 &  38 & 0.34   \\ % 86099817
 FRB20200525C &  339.63 &  34 & 0.36   \\ % 86092282
 FRB20200603B &  295.08 &  42 & 2.68   \\ % 86321776
 FRB20200606A &  723.34 &  47 & 8.22   \\ % 90015951
 FRB20200613A &  348.95 & 104 & 0.63   \\ % 92773515
 FRB20200614A &  348.79 & 104 & 1.27   \\ % 92844954
 FRB20200617A &  475.73 &  61 & 1.18   \\ % 93628004
 FRB20200621C &  364.26 &  34 & 4.77   \\ % 94585529
 FRB20200622A &  223.01 &  29 & 11.21  \\ % 94672522
 FRB20200629C &  363.79 &  43 & 0.64   \\ % 95416492
 FRB20200701A &  625.23 &  77 & 0.23   \\ % 95677738
 FRB20200702C &  201.28 &  46 & 5.41   \\ % 95822946
 FRB20200707A &  218.04 &  84 & 0.07   \\ % 96534808
 FRB20200709C &  363.56 &  43 & 1.75   \\ % 97646351
 FRB20200717A &  337.98 & 135 & 1.27   \\ % 100997459
 FRB20200725B &  302.35 &  50 & 1.39   \\ % 104638972
 FRB20200809G &  221.85 &  29 & 2.75   \\ % 114118424
 FRB20200813D &  190.80 &  53 & 0.03   \\ % 116066865
 FRB20200909A &  221.22 &  29 & \ensuremath{<} 0.1  \\ % 133646258
 FRB20200917A &  883.48 &  74 & 0.73   \\ % 135259857
 FRB20200918A &  314.44 &  26 & 0.12   \\ % 135521375
 FRB20200921A &  465.25 &  31 & 0.23   \\ % 135866445
 FRB20200921B & 1582.12 & 129 & 0.77   \\ % 135856796
 FRB20200930A &  851.58 &  49 & 0.27   \\ % 137003986
 FRB20201008A &  290.26 & 109 & 1.29   \\ % 137628984
 FRB20201015B &  173.79 &  55 & 0.82   \\ % 138368391
 FRB20201017A &  773.68 &  78 & 2.29   \\ % 138618955
 FRB20201030B &  479.80 & 114 & 0.33   \\ % 140210071
 FRB20201031B &  819.71 &  21 & 2.75   \\ % 140464005
 FRB20201125B &  413.71 &  38 & \ensuremath{<} 0.1  \\ % 144722364
 FRB20201128D &  157.88 &  38 & \ensuremath{<} 0.1  \\ % 145086396
 FRB20201129A &   87.86 &  42 & 0.28   \\ % 145207799
 FRB20201203C &  413.50 &  38 & 7.23   \\ % 145654275
 FRB20201204D &  364.25 &  34 & 4.95   \\ % 145781585
 FRB20201205B &  552.46 & 174 & 0.90   \\ % 145838592
 FRB20201219A &  322.20 &  38 & 4.09   \\ % 148108132
 FRB20201225B &  362.74 &  43 & 0.87   \\ % 148980870
 FRB20201225D &  287.96 &  57 & 5.37   \\ % 148957878
 FRB20201228A &  362.91 &  43 & 3.37   \\ % 149540279
 FRB20201230B &  256.13 & 144 & 0.05   \\ % 149825845
 FRB20210104B & 1236.69 &  22 & \ensuremath{<} 0.1  \\ % 150709160
 FRB20210105G &  288.02 &  57 & 2.48   \\ % 150850977
 FRB20210111E &  349.29 & 104 & 1.13   \\ % 151677988
 FRB20210113C &  176.85 &  57 & 1.78   \\ % 152062271
 FRB20210114B &  288.48 &  57 & 0.47   \\ % 152187528
 FRB20210115C &  200.91 &  46 & 2.34   \\ % 152308061
 FRB20210117E &  289.61 &  57 & 5.56   \\ % 152623236
 FRB20210118B &  288.24 &  57 & 9.94   \\ % 152716207
 FRB20210119B &  440.43 &  29 & \ensuremath{<} 0.1  \\ % 152879076
 FRB20210122B &  369.78 &  44 & 0.83   \\ % 153287440
 FRB20210127E &  348.88 & 104 & 2.61   \\ % 153859596
 FRB20210130H &  349.98 & 104 & 49.46  \\ % 154913824
 FRB20210130I &  349.47 & 104 & 13.75  \\ % 154910364
 FRB20210131A &  349.35 & 104 & 1.18   \\ % 155079679
 FRB20210203B &  579.94 &  72 & \ensuremath{<} 0.1  \\ % 155679530
 FRB20210203C &  221.65 &  29 & 0.16   \\ % 155646493
 FRB20210206A &  361.32 & 191 & 0.75   \\ % 156410110
 FRB20210207A &  221.87 &  29 & 4.97   \\ % 156691863
 FRB20210209B &  222.19 &  29 & 2.17   \\ % 157073977
 FRB20210209C &  382.35 &  29 & \ensuremath{<} 0.1  \\ % 157073938
 FRB20210211B & 1090.02 &  76 & 4.46   \\ % 157363005
 FRB20210213A &  482.40 &  46 & 0.05   \\ % 157646917
 FRB20210216B &  301.50 &  50 & \ensuremath{<} 0.1  \\ % 158514696
 FRB20210223A &  531.01 &  43 & 0.99   \\ % 161700760
 FRB20210302A &  349.44 & 104 & 5.85   \\ % 163181014
 FRB20210302C &  221.32 &  29 & 2.60   \\ % 163100809
 FRB20210303B &  349.26 & 104 & \ensuremath{<} 0.1  \\ % 163362088
 FRB20210303F &  510.06 &  51 & 4.41   \\ % 163213672
 FRB20210304A &  348.90 & 104 & \ensuremath{<} 0.1  \\ % 163534005
 FRB20210309D &  134.07 &  32 & 0.50   \\ % 164240257
 FRB20210310A &  135.50 &  20 & 1.55   \\ % 164389739
 FRB20210313B &  414.00 &  38 & 1.59   \\ % 164885944
 FRB20210314A &  413.72 &  38 & \ensuremath{<} 0.1  \\ % 165001685
 FRB20210326B &  413.82 &  38 & \ensuremath{<} 0.1  \\ % 165956452
 FRB20210327A &  415.92 & 140 & 15.40  \\ % 166030118
 FRB20210331A &  417.48 & 140 & 11.61  \\ % 166462622
 FRB20210331C &  414.66 & 149 & 14.13  \\ % 166462644
 FRB20210331D &  415.19 & 140 & 11.17  \\ % 166462575
 FRB20210402B &  349.86 & 193 & \ensuremath{<} 0.1  \\ % 166812476
 FRB20210410C &  301.97 &  50 & 0.74   \\ % 167591075
 FRB20210421E &   87.76 &  42 & 0.24   \\ % 168743856
 FRB20210430G &   87.76 &  41 & 0.14   \\ % 169669688
 FRB20210521C &  349.11 & 104 & 3.67   \\ % 171681248
 FRB20210523A &  348.84 & 199 & 1.65   \\ % 171855709
 FRB20210523C &  532.14 &  41 & 0.87   \\ % 171808929
 FRB20210526B &  382.39 &  29 & 4.57   \\ % 172091258
 FRB20210526D &  411.86 & 131 & 10.66  \\ % 172176403
 FRB20210610B &  694.91 &  50 & \ensuremath{<} 0.1  \\ % 173616504
 FRB20210610C &  876.40 &  21 & 6.72   \\ % 173588081
 FRB20210612B &  579.88 &  72 & 262.75 \\ % 173825813
 FRB20210624A &  413.49 &  38 & 1.00   \\ % 174906271
 FRB20210625A &  349.18 & 104 & 0.54   \\ % 175004577
 FRB20210711A &  349.33 & 199 & \ensuremath{<} 0.1  \\ % 175929272
 FRB20210712A &  348.85 & 104 & 0.01   \\ % 176060009
 FRB20210810C &  694.33 &  50 & \ensuremath{<} 0.1  \\ % 180108339
 FRB20210814B &  349.07 & 104 & \ensuremath{<} 0.1  \\ % 180667327
 FRB20210814C &  348.89 & 104 & \ensuremath{<} 0.1  \\ % 180666196


==> constraints.tex <==
%\newcommand{M_{\odot}}{M_{\odot}}
\section{Constraints}
We calculate the optical depth to lensing in the cosmic web for an FRB at some redshift and brightness. We begin by reviewing the formalism of \citet{sammons2020first} in Sec.~\ref{sec:oneone}. Then, we extend the formalism to consider arbitrary power-law mass functions~\ref{sec:manyone}, and present a formalism for interpreting the results of our search in Sec.~\ref{sec:manymany} and a Bayesian parameter estimation in Sec.~\ref{sec:bayes}. In this writeup we use the following variables:

\begin{center}
\begin{tabular}{r|l|l}
    \textbf{Quantity} & \textbf{Definition} & \textbf{``Typical'' value} \\
    $z_L$  & Redshift of lens & $< 0.5$ \\
    $z_S$  & Redshift of source &  DM$_{eg}$ / (1000 pc-cm$^3$) \\
    $\vec{\Omega}$ & Cosmological parameters & $\Lambda$CDM \\
    $E(z)$ & $H(z) / H_0$ & $\mathcal{O}(1)$ \\
    $m_{min} < m < m_{max}$     & Mass distribution parameters & $10^{-4}-10^2 M_{\odot}$ \\ 
    $R_E(z_L,z_S,m)$    & Einstein radius & 100 light-days \\ 
    $\tau_{min}(m,z_L) $ & Min resolvable time delay & $\approx 1$ ns \\
    $\tau_{max} $ & Max resolvable time delay & $\approx 1$ s \\
    $\sigma(R_E,y_{min},y_{max})$ & Cross section to lensing, & 100 (light-days)$^2$ \\
    $R_{min} < R_{f}$ & Most extreme flux ratio & $\sim 1000$ \\
    $n_c(m)$ & Comoving number density of lenses & Varies \\
    $y_{min}(\tau_{min})$ & Min observable impact parameter $b / R_{E}$ & $\approx 0$ \\ 
    $y_{max}(R_f)$        & Max observable impact parameter $b / R_{E}$ & $\approx 3$ \\ 
    $\tau_L$ & Optical depth to lensing & $\sim 0.01$ \\
\end{tabular}
\end{center}

\subsection{One Lens, One FRB}\label{sec:oneone}
The statistics of gravitational lensing are often times predicted with the formalism of the lensing optical depth, which roughly quantifies the probability that a particular sightline experiences gravitational lensing. For a lens of mass $m$ and redshift $z_L$, we can define a cross section (with units of physical distance squared). 
\begin{equation}
\sigma = \pi R_E^2 (y^2_{max} - y^2_{min})
\end{equation}
In this equation...

\begin{enumerate}
    \item $R_E$ is the Einstein radius:
        \begin{equation}
            R_E^2 = \dfrac{2 R_s D_L D_{LS}}{D_S}
        \end{equation}
    \item $R_s$ is the Schwarzchild radius of the lens.
    \item $D_L$, $D_{LS}$ and $D_S$ are angular diameter distances.
    \item $y_{max}$ is the maximum impact parameter in the lens plane that we are sensitive to. In the case of time-domain microlensing, it is most sensitive to by the maximum detectable flux ratio, $R_f$, via
        \begin{equation}
        y_{max}^2(R_f) = \dfrac{1 + R_f}{\sqrt{R_f}} - 2 = y_{max}^2(1/R_f)
        \end{equation}
        In turn, $R_f$ depends on the SNR of the burst as detected in autocorrelation. $R_f$ is not 5 as suggested in ~\citet{munoz2016lensing}, but it is related to the SNR of the burst and dependent on the details of the correlation algorithm.
    \item $y_{min}$ is the minimum impact parameter in the lens plane that we can resolve. In traditional microlensing studies which directly resolve the images, this is limited by angular resolution, but in our case $y_{min}$ is sensitive to the time delay. If we put a lens at $y = y_{min}$ and the source at $x = 0$, the images pass through the lens plane in two radial positions, given by 
        %
        \begin{equation}
        y_{\pm} = \dfrac{y_{min}}{2}\pm \dfrac{\sqrt{y_{min}^2 + 4}}{2}
        \end{equation}
        %
        Evaluating the time delay potential at these two points in the lens plane implicitly defines $y_{min}(\tau_{min},m,z_L)$: 
        %
        \begin{equation}
        \tau_{min} < \tau_+ - \tau_- = \dfrac{2 R_s(1 + z_L)}{c} \left[ \dfrac{1}{2}(y_{min}\sqrt{y_{min}^2 + 4}) - \log\left(\dfrac{y_{min} - \sqrt{y_{min}^2 + 4}}{y_{min} + \sqrt{y_{min}^2 + 4}}\right) \right]
        \end{equation}
\end{enumerate}

Finally, the optical depth due to lensing, for one lens of mass $m$ at some arbitrary redshift $z_L$ and one FRB at redshift $z_S$, is given by integrating the cross section multiplied by the comoving number density along the line of sight $n_c(m) = n_{c,0} \delta(m = m_0)$.
 Since we're considering a monochromatic mass distribution, a better way to write the same equation is to think of what we just called $\tau_L$ as a differential optical depth to lenses of mass $m$. 
\begin{equation}
    \dfrac{d\tau_L}{dm}(m,z_S) = \int n_c(m) \sigma~d\chi = \int_0^{z_S} n_c \sigma\dfrac{d\chi}{dz}~dz = D_H \int_0^{z_S} \dfrac{n_c \sigma(z_L,z_S,m,\tau_{min},R_f) }{(1 + z_L) E(z_L)}~dz_L
\label{eq:basic}
\end{equation}

Integrating over $m$ gives us

\begin{equation}
    \tau_L(m_0,z_S) = \int n_{c,0} \sigma~d\chi = \int_0^{z_S} n_{c,0} \sigma\dfrac{d\chi}{dz}~dz = D_H \int_0^{z_S} \dfrac{n_c \sigma(z_L,z_S,m_0,\tau_{min},R_f) }{(1 + z_L) E(z_L)}~dz_L
\label{eq:basic_int}
\end{equation}

\begin{figure}
    \begin{center}
    \includegraphics[width = 0.5\textwidth]{./sammons_2020.png}
    \caption{Reproducing Sammons et al. figure with our code to check that it calculates optical depths correctly.}
    \end{center}
\end{figure}

\subsection{Many Lenses, One FRB: The Microlens Mass Function}\label{sec:manyone}
Now that we have defined the optical depth towards a delta-function population of mass $m$ (more precisely, the differential optical depth $d\tau/dm$), we generalize Eq.~\ref{eq:basic_int} to the more realistic situation where we have an diverse population of scatterers, each endowed with its own cross section. In this case we must integrate Eq.~\ref{eq:basic} over the population of lenses. The universe is full of lenses of different masses, and $\tau_L$ depends on the lens mass through $R_E$ and $y_{min}$.

The microlens mass in turn is drawn from a (Salpeter, Kroupa, etc.) mass function. So, the resulting $\tau_L$ for a population of lenses depends on the microlens mass function. \citet{shetty2014salpeter} suggests on the basis of galaxy kinematics that at $z \approx 1$, a Salpeter mass function (a power law) does the job well.\\

Mass functions are typically quoted as a volumetric number density per unit mass. For extragalactic astronomy, it makes sense to parameterize mass functions as a comoving volume number density (rather than a physical). While the physical density increases $\propto (1 + z)^3$, the comoving number (and mass) density remain constant. 

\begin{equation}
    dn_c = n_0 \left( \dfrac{m}{M_{\odot}}\right)^{-\gamma} \left( \dfrac{dm}{M_{\odot}} \right)
\end{equation}

where the constant $n_0$ has units of number per comoving volume. The comoving mass density of lenses within a certain mass range is

\begin{align}
    \dfrac{dm}{dV_c}= \int_{m_{min}}^{m_{max}} m~\dfrac{dn_c}{dm}~dm &= n_0 \int_{m_{min}}^{m_{max}} m \left( \dfrac{m}{M_{\odot}}\right)^{-\gamma} \left( \dfrac{dm}{M_{\odot}} \right) = n_0 M_{\odot} \int_{m_{min}/M_{\odot}}^{m_{max}/M_{\odot}} \left( \dfrac{m}{M_{\odot}}\right)^{1-\gamma} d\left( \dfrac{m}{M_{\odot}} \right) \\
&= \dfrac{n_0M_{\odot}}{2-\gamma} \left[ \left(\dfrac{m_{max}}{M_{\odot}}\right)^{2-\gamma} - \left(\dfrac{m_{min}}{M_{\odot}}\right)^{2-\gamma} \right]
\end{align}

This can be matched to the expected cosmological abundance of microlenses, which gives us a handle on the cosmology. We ignore the effects of large-scale structure, and assume a homogeneous and fixed (comoving) density of microlenses parameterized in terms of the (physical) critical density as

\begin{align}
    \dfrac{dm}{dV_c} = \dfrac{dm}{dV} \dfrac{dV}{dV_c} &= \dfrac{3 H_0^2 \Omega_{lens}}{8\pi G} \times (1 + z)^3
\intertext{where we used $\dfrac{dV}{dV_c} = (1 + z)^3$. The cosmologically-expected mass function is then}
    dn(m,z_L,\vec{\Omega}) &= \boxed{\dfrac{3 H_0^2 (1 + z_L)^3 \Omega_{lens} (2 - \gamma)}{8\pi GM_{\odot}}
    \left[ 
        \left(
            \dfrac{m_{max}}{M_{\odot}}
        \right)^{2-\gamma} 
        - 
        \left(
            \dfrac{m_{min}}{M_{\odot}}
        \right)^{2-\gamma} 
    \right]^{-1} 
    \left( \dfrac{m}{M_{\odot}}\right)^{-\gamma} \left( \dfrac{dm}{M_{\odot}} \right) }
\label{eq:cosmo_imf}
\end{align}

The optical depth for one source given such an ensemble of lenses is as follows (compare with Eq.~\ref{eq:basic}). I have written down all the parameter dependences, abbreviating the minimum and maximum lag bins $\tau_{min},\tau_{max}$ as $\tau_j$, and the minimum and maximum masses in a mass bin $m_k$ as $m_{min,k},m_{max,k}$.
\begin{align}
\tau_L (z_S,m_{k},R_{max},\tau_j,\vec{\Omega}) &= \\ \int_{m_{min,k}}^{m_{max,k}} dm \int_0^{z_S} dz_L& \dfrac{R_H}{(1 + z_L) E(z_L,\vec{\Omega})} \times \\
    & \dfrac{dn}{dm}(m,z_L,\vec{\Omega}) \times \\ 
& \sigma(m,\vec{\Omega},z_L,R_{max},\tau_j)\\
\label{eq:tau_imf}
    \intertext{To rewrite things a bit clearer, we can consolidate powers of $1 + z_L$:}
    \tau_L (z_S,m_{k},R_{max},\tau_j,\vec{\Omega}) &= \\ \int_{m_{min,k}}^{m_{max,k}} dm \int_0^{z_S} dz_L& \dfrac{R_H (1 + z_L)^2}{E(z_L,\vec{\Omega})} \times \\
    & \dfrac{dn_c}{dm}(m,\vec{\Omega}) \times \\ 
& \sigma(m,\vec{\Omega},z_L,R_{max},\tau_j)
\end{align}

\subsection{Many Lenses, Many FRBs}\label{sec:manymany}
Now that we have defined the optical depth to one FRB, we can consider stacking events by stacking their optical depths. In the conventional definition of optical depth, scatterers deflect the original radiation, and the survival probability of a single ray passing through a medium of optical depth $\tau$ is $P(\textrm{no interaction}) = \exp(-\tau)$. This means that $P(\textrm{scatter}) = 1 - \exp(-\tau) \approx \tau$. If there are many sightlines indexed by $s$, the expected number of
encounters is $\sum_{s} \tau_s$.

For each FRB source $s$ and lag bin $j$, we measure $DM_s$ and $G(\tau)$ for a large range of lags. We can translate the $DM_s$ to $z_{s}$ assuming the Macquart relation holds. To interpret $G(\tau)$, we separate it into different lag bins. If we carefully interpret the autocorrelation functions, we can deduce for source $s$ in lag bin $j$ the number of excursions we saw $n^{sj}$ as a function of the flux ratio threshold $R^{sj}_f$. We convert the ACF to flux ratio units,

\begin{equation}
    R^{sj}_f(\tau) = \dfrac{G_{on}(\tau = \tau) - G_{off}(\tau = \tau)}{G_{on}(\tau = 0) - G_{off}(\tau = 0)}.
\end{equation}

or equivalently, into units where noise has unit variance.

Fora given threshold $R_f^{sj}(\tau)$, we can then simply count the number of lensing events. There are many ways to do this: you could take things directly from the excursion histogram, but you don't even need to do that. The $n^{sj},R^{sj}_f$ plane is just a convenient way to parameterize our interpretation. To illustrate this, consider the following three possibilities in order from most to least optimistic.

\begin{enumerate}
    \item For every sightline the universe is swimming with lenses. Coincidentally, we found exactly one lens in every single lag bin for one burst and there is no RFI. In this case, we would declare that 

    \begin{equation}
        (n^{sj} = 1,R^{sj}_f) = (1, \max_{\tau \in [\tau_{j,min},\tau_{j,max}]}(R^{sj}_f(\tau))
    \end{equation}

        for each lag bin in that burst, and report the $R^{sj}_f$ of the lensing candidate to estimate the optical depth.

    \item There are no lenses (null hypothesis), and no RFI or backgrounds. But on the bright side, we were sensitive to flux ratios as extreme as $R^{sj}_f$ taken as the maximum value in each lag bin!  

        \begin{equation}
            (n^{sj}, R^{sj}_f) = (0,\max_{\tau \in [\tau_{j,min},\tau_{j,max}]}(R^{sj}_f(\tau)))
        \end{equation}

    \item There are no lenses but lots of backgrounds. We apply vetoes (checking both polarizations, checking the mocks for excursions), and remove from consideration the excursions that did not pass those checks. We eliminate several of the biggest excursions (let's say there are ten of them). We choose the null hypothesis that there were no lenses. We would choose the eleventh largest value of $R^{sj}_f(\tau)$ within a lag bin as our sensitivity threshold, and choose $n^{sj} = 0$ for each lag bin.

        \begin{equation}
            (n^{sj}, R^{sj}_f) = (0,\text{eleventh largest }(R^{sj}_f(\tau)))
        \end{equation}

\end{enumerate}
So, a combination of a flux ratio $R^{sj}_f$ and an interpretation $n^{sj}$ parameterize our interpretation of our data. 
We can combine FRBs by calculating the ``all-sky'' rate of lensing events

\begin{align}
    n^{j} = &\sum_s n^{sj} \\
    \intertext{as well as the ``all-sky'' optical depth}
    \tau^\ast_{L}(m_{k},\tau_j,\vec{\Omega}) = & \sum_{s} \tau_L (z_s,m_{k},R^{sj}_{max},\tau_j,\vec{\Omega})
\end{align}

where we sum the optical depth over all sources $s$, and plug in $R^{sj}_f$ numbers from above and $z_S$ from the Macquart relation. 

\subsection{Bayesian Parameter Estimation}\label{sec:bayes}
Having combined the information from an ensemble of FRBs, how do we translate this into statistical upper limits on microlensing? We can combine lag bins by using maximum likelihood estimators for each lag bin and treating them as independent experiments. The likelihood as a function of cosmological parameters $\vec{\Omega}$ and lens mass bin $m_{min},m_{max}$ (which we abbreviate as $ m_{k}$) can be written down a la Bayes:~\citep{zyla2020review}. We are interested in the posterior distribution of cosmological parameters given the total number of lenses that we saw $n^j$ and our estimate of the all-sky optical depth $\tau^{\ast~j}_{L}$. The optical depth has a mass bin dependence too, but we will suppress it for the sake of clarity.

\begin{align}
    P(\underbrace{\vec{\Omega}}_{cosmology}|\underbrace{n^j,\tau_L^{\ast j}}_{data}) 
    &\propto \underbrace{P(\vec{\Omega})}_{prior} 
        \mathcal{L}
    \intertext{
        where $\mathcal{L}$, the likelihood, refers to the probability of getting the data we observed given some underlying parameters of interest. Let's take the prior to be uniform in $\vec{\Omega}$. In our case, $\mathcal{L}$ is a product of the likelihoods from different lag bins $j$. In addition, the likelihood is Poissonian: the number of lensing events in a lag bin $n^{j}$ is integer-valued, $<<1$, and therefore largely independent.
    }
    \mathcal{L} &= \prod_{j} P(\underbrace{\tau_L^{\ast j},n^j}_{data} | \underbrace{\vec{\Omega}}_{cosmology}) \\
    \intertext{
        Another way of saying this is that the log-likelihood is summed over lag bins $j$.
    }
    -\log\mathcal{L}(\vec{\Omega}) &= \sum_{j} \left[ \tau^{\ast j} - n^{j} + n^{j} \ln( n^{j} / \tau^{\ast j}) \right]
    \intertext{In the useful special case that $n^j = 0$ everywhere this simplifies to}
                                   &= \sum_{j} \tau^{\ast j} 
\end{align}

Calculating the likelihood as a function of $\Omega_{microlens}$ will get us an inference on what its value is as a function of mass range; repeating for different mass ranges will allow us to set upper limits on the abundance of microlenses. We could do the same with other mass function parameters such as $\gamma$, but I am not sure they will be very sensitive to the statistics here.

\section{Plugging in Numbers for one FRB}
For the super-bright FRB 65547659, with a SNR optimized DM = 454.56, we have a burst SEFD of $\sigma_s^2 / \sigma_n^2 \approx 15000 / 2500 = 20$ (eyeballed from the graph):
\begin{figure}
    \begin{center}
    \includegraphics[width = 0.49\textwidth]{./chime_2021.png}
    \includegraphics[width = 0.49\textwidth]{./constraints_abcd.png}
    \includegraphics[width = 0.49\textwidth]{./constraints_ab.png}
    \includegraphics[width = 0.49\textwidth]{./constraints_c.png}
    \end{center}
    \caption{Top left: Constraints like those from~\citep{sammons2020first} for FRB 65547659 alone. Top right: Constraints for full sample, without removing any wave effects, in the slice $f_{DM} = 1$. Bottom left: Model-independent component of constraints. Bottom right: Model-dependent component of constraints.}
\end{figure}

Its duration is about 100 $\mu s$. Therefore, $M' = 100 / 2.56 = 40$, and we have a flux limit from Eq.~\ref{eq:radiometer_coherent} corresponding to 

\begin{align}
    R_f = \varepsilon^2 &> Z^2 \times \dfrac{\sigma_n^4}{\sigma_s^4}\dfrac{(1 + \dfrac{\sigma_s^2}{\sigma_n^2})}{NM'} \\
    R_f &\approx 2.3\times 10^{-5} \\
    100~\textrm{ms} \gtrsim \tau &\gtrsim 50~\textrm{ns} \\
    z_S &\approx 0.445 \\
\end{align}

If we assume $R_f$ is the same for all different delays, we may place a constraint in the same way that ASKAP does for their bursts, with superlative numbers! This is shown in the figure above.



==> pfb.tex <==
Working in baseband space is an excellent way to concentrate the signal as much as possible, but for the lens search it is necessary to return to timestream space to autocorrelate the voltage signal. This is accomplished by a process called polyphase filter bank inversion~\cite{mcsweeney2020mwa,morrison2020performance} in which data from many frequency channels is synthesized into a high time-resolution timestream. This inversion is in principle lossless, but the phased-array beamforming and coherent dedispersion--both of which are necessary steps for data reduction--have introduced noise into the data which makes the exact inversion an ill-conditioned inverse problem.

We solve this problem with a novel PFB inversion method which we refer to as the phase-averaged circulant method. We take the average frequency response over each of the 2048 filters in the filter bank and assume periodic (circulant) boundary conditions to the timestream. This is a good approximation when the input signal is stationary on timescales less than the duration of a PFB tap (2.56 $\mu$s). In this approximation, the eigenmodes of the forward PFB operation are complex exponentials,
enabling an FFT implementation of the inversion. The output of this operation is a timestream $E(t)$, which is the whitened electric field as a function of time.


==> pipeline.tex <==

CHIME/FRB Baseband system does not save raw voltage data. The voltage data from the sky undergoes the following processing stages before being processed with our search pipeline. 
\begin{enumerate}
    \item Voltage data is band-passed to 400-800 MHz. An ADC at 800 MHz undersamples the voltage data up to its Nyquist frequency of 400 MHz. A scaling is applied to each antenna to minimize quantization distortions (these are the so-called digital gains). 
    \item A polyphase filter bank (PFB) is applied to the quantized voltage data in the so-called F-engine.
    \item Channelized data grouped by antenna in the F engine is regrouped by frequency in a so-called corner-turn operation which passes data to the X engine, which performs correlation  over 1024 frequency ``channels'' of bandwidth 390 kHz. 
    \item After grouping data by frequency, 4+4 real+imaginary bits of baseband data are written to disk upon a trigger from the real-time FRB detection system. Some frequency channels are not present, or are removed because of the presence of strong RFI.
    \item To improve sensitivity towards a certain sky direction we form tied-array beams and perform coherent de-dispersion on the baseband data.
\end{enumerate}
At the end of this procedure, we have concentrated our FRB signal by coherently summing over antennas, concentrating the signal over different antennas by a factor of 1024, and coherent dedispersion on the beamformed baseband, which concentrates the signal in time by a factor of $\sim 10$.



==> rf.tex <==
The whitened, band-integrated ``flux'' as a function of time can be written $E^2(t)$, and the fluence can be measured by summing over time samples. 
To improve the sensitivity of the correlation, we also use a window function to exploit the temporal structure of the FRB. After coherent de-dispersion and RFI removal in baseband space, we construct the window function by summing over channels and smoothing the resulting light curve with a Gaussian whose width $\sigma$ is set by the variability timescale of the FRB. Finally, the autocorrelation code
computes

$$G(\tau) = \sum_t E(t) E(t + \tau) W(t)$$

as a function of trial delay $\tau$. From the correlator output we can extract the magnification ratio as a function of lag. This conversion is done as follows. We first define the quantity
%
$$S_W(\tau) = \sum_t E^2(t) W(t + \tau).$$
%
and choose the normalization of $W$ such that $S_W(0)$ is the fluence of the burst. We call this quantity the lag-fluence. It is equivalent to the fluence at zero lag, where it is at its maximum, but as $\tau$ increases the window gets misaligned with the light curve $S_W(\tau)$ decreases. Eventually the window moves to delays longer than the pulse duration, and $S_W(\tau) \to 0$.
Our correlator computes 
%
$$G(\tau) = \sum_t E(t) E(t + \tau) W(t).$$
%
Suppose that the timestream $E(t)$ contains a second image corresponding to a putative lens signal, with a flux magnification ratio of $\epsilon^2 < 1$. In the regime of coherent lensing (see Section~\ref{sec:decoherence}), semiclassical (or eikonal~\cite{jow2020wave}) optics allows us to model the electric field from the second image as $E'(t) = \epsilon E(t - \tau_{lens})$. In this limit, $E'$ and $E$ correlate with each other when they are temporally aligned $(\tau = \tau_{lens})$, yielding a peak in the autocorrelation function of magnitude
%
$$G(\tau_{lens}) = \epsilon S_W(0)$$
%
The autocorrelation peak at zero lag is boosted as well. After subtracting the background from the system temperature, the zero lag peak height is
$$G(0) = S_W(0) + \epsilon^2 S_W(\tau_{lens})$$
We calculate
$$\mathcal{R}(\tau) = G(\tau) / G(0) = \dfrac{\epsilon}{1 + \epsilon^2 S_W(\tau_{lens})/S_W(0)}.$$
%
Solving for $\epsilon$ gives us 
$$
\epsilon(\tau) = 
\begin{cases}
    \dfrac{S_W(0)}{S_W(\tau_{lens})\mathcal{R}(\tau)} - \mathcal{R}(\tau) - 2\mathcal{R}(\tau)^3\dfrac{S_W(\tau_{lens})}{S_W(0)} \\ \mathcal{R}(\tau) + 2 \dfrac{S_W(\tau_{lens})}{S_W(0)} \mathcal{R}(\tau)^3 
\end{cases}
$$

The former solution is unphysical and diverges as $S_W(\tau_{lens}),\mathcal{R}(\tau) \to 0$. Furthermore, for lags larger than a few nanoseconds, $|\mathcal{R}(\tau)| < 0.05$, making the $\mathcal{R}^3$ term negligible. Thus the lens magnification ratio is to leading order
%
$$\epsilon^2 = |G(\tau) / G(0)|^2 + \mathcal{O}(|G(\tau) / G(0)|^4).$$
%

==> scratch/oqe.tex <==
\section{Correlation Algorithm}
We are fundamentally interested in a quadratic function of the data. But we can make a lot of progress by using a subframe averaged circulant-PFB inverse to invert baseband data $F_{mk}$ back to a pseudo-timestream to circumvent segmentation loss over the frame axis, which reduces our sensitivity by $\mathcal{O}(25\%)$. We are working on an optimal quadratic estimator for the correlation function $G(d)$ to remove the PFB artifacts. After having conducted a literature search, I found a few references on software correlation with a PFB. \cite{morrison2020performance} performs correlation on an oversampled PFB (one where the channels overlap) by going into frequency space, extracting the center parts of each channel, calculating the cross-power spectrum, and calculating the correlation function by inverse transform. This approach works best for oversampled PFBs, where all the information is preserved, and not for critically-sampled PFBs in which the channels have very low leakage (and therefore little redundancy). \cite{mcsweeney2020mwa} performs correlation with the synthesis filter technique, designing a $N$ tap long function which when convolved with baseband data and FFT'ed gives an accurate reconstruction of the timestream. If a ``perfect reconstruction filter bank'' is used for the forward PFB it can be inverted if all channels are present. Practically, this is unfortunately not the case with triggered VLBI observations, where certain channels will be masked due to RFI and where data dumps are not of a homogenous rectangular shape. \texttt{DiFX} uses a basic ``channel-by-channel'' correlation algorithm: I could find no details of a non-trivial correlation algorithm, and the code in \texttt{https://svn.atnf.csiro.au/difx/master\_tags/DiFX-2.3.1/mpifxcorr/src/core.cpp} seems to indicate that DiFX simply performs complex multiply accumulation of baseband data points.

First, let's review the optimal quadratic estimator recipe for the CMB.

\subsection{CMB}
In the CMB, the input is a skymap comprised of pixels $x_i$ and the output of the meat grinder is the angular power spectrum $C_\ell$. Tegmark makes the guess that the $C_{\ell}$ is quadratic in the data: $x_i x_j$, using the observation that $\langle x_i x_j \rangle$ can be decomposed as follows:
\begin{align}
    \langle x_i x_j \rangle = N_{ij} + &\sum_{\ell} C_{\ell} P^\ell_{ij}\label{eq:P_ell_def}
    \intertext{where $\langle x_i x_j \rangle$ denotes the two point function of the data, $N_{ij}$ is the noise covariance matrix, and a linear combination of basis functions $P^\ell_{ij}$ whose coefficients are the $C_\ell$'s. The optimal estimator is}
    C_\ell &= \dfrac{1}{2}F^{-1}_{\ell \ell'} [(x_i (C^{-1})_{ik} P^{\ell'}_{km} (C^{-1})_{mj} x_j) - \mathrm{Tr}[(C^{-1})_{pq} P^{\ell'}_{qr}]
    \intertext{where $x_i$/$x_j$ are the data, where $(C^{-1})_{ik}$ is the inverse covariance matrix of the data, where $P^{\ell'}_{km}$ is a list of matrices, one for each value of $\ell$, that is symmetric in its two indices $k,m$.}
    \intertext{$F_{\ell \ell'}$ is the Fisher matrix, and can be interpreted as}
    F_{\ell \ell'} &= \dfrac{\partial^2 \ln \mathcal{L}}{d\ell d\ell'} \\
    \intertext{To estimate $F_{\ell \ell'}$ we use}
    F_{\ell \ell'} &= \dfrac{1}{2} \mathrm{Tr}[P^{\ell}_{ij} (C^{-1})_{jk} P^{\ell'}_{kl} (C^{-1})_{lm} ]
    \intertext{This gives us an ingredient list: to get an optimal quadratic estimate of $C_{\ell}$, we need to compute the inverse covariance of the data $C^{-1}_{ij}$, and a list of matrices $P^{\ell}_{ij}$ (these can be thought of as the gradient of the two-point function with respect to the parameters to be estimated). The actual form of the estimator is}
\end{align}
\begin{equation}
    \boxed{\hat{C_\ell} = (F^{\ell \ell'})^{-1}\left[\sum_{ijkl} x_i (C^{-1})_{ij} P^{\ell'}_{jk} (C^{-1})_{kl} x_l \right]} 
\end{equation}
\subsection{FRB}
We make an analogy with cross correlation functions using the fact that in FRB lensing we are interested in the voltage autocorrelation function--a quadratic function--of the data. The estimator has the same form:

\begin{equation}
    \boxed{\hat{G^d} = (F^{d d'})^{-1}\left[\sum_{ijkl} B_i (C^{-1})_{ij} P^{d}_{jk} (C^{-1})_{kl} \overline{B_l} \right]} 
\end{equation}

where the baseband data, $B$, are derived from raw voltages $v_i$ by a polyphase filter bank.
\begin{align}
    B_{mk} &= \sum_{j = 0}^{\infty} W[j - Nm] v[j] \exp(2\pi i j k / N)
    \intertext{with}
    W[q] &= \sin^2\left(\dfrac{\pi q}{4N-1}\right)j_0\left(\dfrac{\pi(q-2N)}{N}\right)
    \intertext{for $0 \leq q < 4N$ and $0$ otherwise.}
\end{align}
If the PFB were the only effect applied to FRB baseband data, we would never need to consider the optimal quadratic estimator approach, because of the circulant PFB inverse algorithm which can quickly and robustly invert $F_{mk} \to v_j$. However, there are a number of other operations applied to baseband data specific to FRB detection are much more difficult to undo in post-processing. Instead of attempting to undo the full signal processing chain, we should look for an algorithm that has some hope of preserving our observable.
The forms of corruption that baseband data undergo can be grouped into three classes of mathematical operations: first, the data are rolled by a different number of frames $m$ in each frequency channel, and random frames are zeroed out. Second, each channel gets upchannelized, and a random unitary transfer function is applied. Third, each channel can be multiplied by a complex gain. We will explain these operations in the context of actual FRB science later--for now, just accept that these operations cannot be trivially undone.
%
Let's find the form of the $P^\ell_{(i)(j)}$ by writing the two-point function of the data as in the left hand side of Eq.~\ref{eq:P_ell_def}. We introduce the known matched filter $h_m$ and instrumental response $S_k$ (taking into account missing frequencies). Letting the overline denote complex conjugation we write
%
\begin{align}
h_m S_k\langle B_{mk} \overline{B_{m' k'}} \rangle = \sum_d G^d P^d_{mk~m'k'} \\
\langle B_{mk} \overline{B_{m' k'}} \rangle = \sum_{j,j' = 0}^{\infty,\infty} W[j - Nm] W[j' - Nm'] &\exp(2\pi i (j k - j' k') / N) \langle v[j] v[j'] \rangle
\intertext{We are summing over the $j,j'$ square which has side length $NM$. We can change coordinates to a diagonal/anti-diagonal coordinate system by defining}
j &= \dfrac{\alpha + \delta}{2} \qquad \qquad j' = \dfrac{\alpha - \delta}{2}\\
\langle B_{mk} \overline{B_{m' k'}} \rangle = \sum_{\delta= - NM}^{\delta = +NM} \sum_{\alpha = \delta}^{\alpha = NM - \delta} &W[\dfrac{\alpha + \delta}{2} - Nm]W[\dfrac{\alpha - \delta}{2} - Nm'] \\
\times & \exp(\dfrac{2\pi i}{2N}((\alpha + \delta) k - (\alpha - \delta) k') \\
\times & \left\langle v\left[\dfrac{\alpha + \delta}{2}\right] v\left[\dfrac{\alpha - \delta}{2}\right] \right\rangle
\intertext{We can break up the exponential in this convenient coordinate system.}
\exp\left(\dfrac{2\pi i \alpha (k - k')}{2N}\right) \exp\left(\dfrac{2\pi i \delta (k + k')}{2N}\right) &\leftarrow \exp(\dfrac{2\pi i}{2N}((\alpha + \delta) k - (\alpha - \delta) k')
\intertext{Since the data is assumed to be linear time invariant, we substitute}
G^d \delta(d = \delta) &\leftarrow\left\langle v\left[\dfrac{\alpha + \delta}{2}\right] v\left[\dfrac{\alpha - \delta}{2}\right] \right\rangle
\intertext{Writing the whole thing again we get}
\langle B_{mk} \overline{B_{m' k'}} \rangle = \sum_{\delta= -  NM}^{\delta = +  NM} \exp\left(\dfrac{2\pi i \delta (k + k')}{2N}\right) \sum_{\alpha = \delta}^{\alpha = NM - \delta} &W[\dfrac{\alpha + \delta}{2} - Nm]W[\dfrac{\alpha - \delta}{2} - Nm'] \\
\times & \exp\left(\dfrac{2\pi i \alpha (k - k')}{2N}\right)  \\
\times & G^d \delta(d = \delta)
\intertext{The Kronecker delta function and the sum over $\delta$ hate each other and challenge each other to a duel. They kill each other. We are left with a sum over $\alpha$.}
= \sum_{\delta= -  NM}^{\delta = + NM}  G^d \delta(d = \delta) \exp\left(\dfrac{2\pi i d (k + k')}{2N}\right) \sum_{\alpha = d}^{\alpha = NM - d} &W[\dfrac{\alpha + d}{2} - Nm]W[\dfrac{\alpha - d}{2} - Nm'] \\
\times & \exp\left(\dfrac{2\pi i \alpha (k - k')}{2N}\right) 
\intertext{This expression is finallly of the form $x_i x_j = \sum_{d} G^{d} P^d_{ij}$, which allows us to identify the full expression for the gradient:}
\end{align}
\begin{equation}
    \boxed{P^{d}_{mk~m'k'} = \exp\left(\dfrac{2\pi i d (k + k')}{2N}\right) \sum_{\alpha = d}^{\alpha = NM - d} W[\dfrac{\alpha + d}{2} - Nm]W[\dfrac{\alpha - d}{2} - Nm'] \exp\left(\dfrac{2\pi i \alpha (k - k')}{2N}\right)}
    \label{eq:pd_full}
\end{equation}
A significant computational and conceptual simplification becomes possible when we project $P^{d}_{mk~m'k'} \to P^{d}_{mk~m'k'} \delta_{k k'}$: the ``no leakage'' approximation, which is good to about a part in 1/N.
\begin{align}
     P^{d}_{mk~m'k'} &= \exp\left(\dfrac{2\pi i kd }{N}\right) \sum_{\alpha = d}^{\alpha = NM - d} W[\dfrac{\alpha + d}{2} - Nm]W[\dfrac{\alpha - d}{2} - Nm']
     \intertext{Substituting $\alpha' = \alpha  - d - 2 N m'$ the limits become}
     \alpha' &= - 2 N m' \\
     \alpha' &= (NM - d) - d - 2 N m'\\
     P^{d}_{mk~m'k'} &= \exp\left(\dfrac{2\pi i kd }{N}\right) \sum_{\alpha = -2 N m'}^{\alpha = NM - 2d - 2 N m'} W[\alpha'/2 + d + N(m' - m)]W[\alpha' / 2]
     \intertext{Noting that the sum is only a function of $d - N (m  - m')$ (since the limits can be extended to infinity, we write this as}
     P^{d}_{mk~m'k'} &= \delta_{k k'} \exp\left(\dfrac{2\pi i kd }{N}\right) K[d + N (m'  - m)]
     \intertext{A nice property of this form is that it is symmetric in $m$ and $m'$. If we had used $\alpha' = \alpha + d - 2 N m$ we would get}
     P^d_{mk~m'k'} &= \delta_{k k'} \exp\left(\dfrac{2\pi i kd }{N}\right) \sum_{\alpha' = 2(d - Nm)}^{\alpha' = N(M - 2m)} W[\alpha'/2 - d - N(m' - m)]W[\alpha' / 2]
     \intertext{which we recognize as}
     P^d_{mk~m'k'} &= \delta_{k k'} \exp\left(\dfrac{2\pi i kd }{N}\right) \sum_{\alpha' = 2(d - Nm)}^{\alpha' = N(M - 2m)} K[-(d + N(m' - m))]
\end{align}

The other ingredient we need is the data covariance matrix. Since $B_{mk}$ has zero mean, the covariance of $B_{mk}$ is
\begin{equation}
    \boxed{\textrm{Cov}(B_{mk}) = \langle B_{mk} \overline{B_{m'k'}} \rangle = \sum_{d} G^d P^d_{mk~m'k'}} \approx P^0_{mk~m'k'}
    \label{eq:cov}
\end{equation}
because the autocorrelation will be dominated by the zero lag term. We could add in more lags if we knew the channel mask function, but maybe $P^0$ is robust enough for now. The last intermediate product is writing down an expression for the Fisher matrix
\begin{align}
F_{d d'} &= \dfrac{1}{2} \mathrm{Tr}[P^{d}_{ij} (C^{-1})_{jk} \overline{P^{d'}_{kl} (C^{-1})_{lm}}]
\intertext{where the complex conjugate forces the Fisher information needs to be positive semidefinite, or else the likelihood function does not have a maximum! In the limit that the covariance matrix is the identity, this becomes}
F_{d d'} &= \dfrac{1}{2} \mathrm{Tr}[P^{d}_{ij} \overline{P^{d'}_{jk}}]
\intertext{expanding the indices we get}
&= \dfrac{1}{2}\mathrm{Tr}[\sum_{m'k'} P^{d}_{mk~m'k'} \overline{P}^{d'}_{m'k'~m''k''}] \\
\intertext{To trace over a matrix is to set its indices equal, insert a delta function, and sum over both indices. Tracing over $m,m'',k,k''$ means we impose $m = m''$ and $k = k''$, putting in four sums.}
= \dfrac{1}{2}\sum_{m,m',m''} \sum_{k,k',k''} &\left[ \delta_{m m''} \delta_{k k''} P^{d}_{mk~m'k'} \overline{P}^{d'}_{m'k'~m''k''}\right] \\
= \dfrac{1}{2}\sum_{m,m',m''} \delta_{m~m''} \sum_{k,k',k''}  &\delta_{k k'} \exp\left(\dfrac{2\pi i kd }{N}\right) K[d - N (m  - m')] \\
\times &\delta_{k' k''} \exp\left(-\dfrac{2\pi i k'd' }{N}\right) K[d' - N (m'  - m'')] \\
= \dfrac{1}{2}\sum_{m,m',m''} \delta_{m~m''} \sum_{k,k',k''}  &\delta_{k k'} \exp\left(\dfrac{2\pi i kd }{N}\right) K[d - N (m  - m')] \\
\times &\delta_{k' k''} \exp\left(-\dfrac{2\pi i k'd' }{N}\right) K[d' - N (m'  - m'')] \\
\intertext{Now, we start collapsing the sums. We can do the sum over $k''$ and $k$ by collapsing the delta functions.}
= \dfrac{1}{2}\sum_{k'}  \exp\left(\dfrac{2\pi i k' (d - d') }{N}\right) &\sum_{m,m',m''} \delta_{m~m''}   K[d - N (m  - m')]K[d' - N (m'  - m'')] \\
\intertext{We can also sum over $k'$ from $0$ to $N-1$. This gives the periodic Dirichlet kernel in $d - d'$ (an analytic continuation of the $N$-periodic Kronecker delta function.}
\sum_{k'}  \exp\left(\dfrac{2\pi i k' (d - d') }{N}\right)&= D(d - d') = \begin{cases} 
      N & d - d' = mN \\
      0 & d - d' \in \mathbb{Z}
   \end{cases} \\
F^{d d'}= \dfrac{1}{2} D(d = d') \sum_{m,m',m''} \delta_{m~m''} & K[d - N (m  - m')]K[d' - N (m'  - m'')] \\
\intertext{Now we sum over $m''$}
= \dfrac{1}{2} D(d - d') \sum_{m,m' } & K[d - N (m  - m')]K[d' - N (m'  - m)]
\intertext{If we actually wrote out this enormous matrix $F^{dd'}$ we would see that it is quite sparse because of the Dirichlet kernel. Two lags, $d$ and $d'$, are only coupled together if they differ by an integer number of frames. If we set $d - d' = N \Delta m$ (i.e. the values which are nonzero), then $D(d-d') = N$ and this simplifies to}
= \dfrac{1}{2} N \sum_{m,m' } & K[d' + N(\Delta m + m' - m)]K[d' - N (m'  - m)]
\intertext{This is a function only of $\Delta m$ and $d'$. Letting $M'' = N(m' - m)$}
= \dfrac{1}{2} N \sum_{M''} & K[d' + N \Delta m + M'')]K[d' - M'']
\intertext{This does not appear to be the convolution of $K$ with itself, which may be surprising. With some re-indexing it may be more clear.}
\end{align}

\subsection{What happens to baseband data}
During $N^2$ calibration, each antenna signal gets phased up towards some nominal delay center on the sky $\sim 30$ degrees away from the original delay center. Up to a segmentation loss factor on the order of $\tau = 300\mathrm{ns} \times \sin(30^\circ)/2.56\mathrm{\mu s}\sim 10\%$, we can think of this cable delaying process as happening prior to PFB channelization (though in practice it happens afterwards). There are other things too that I haven't listed yet.




==> xf.tex <==
\section{Sensitivity of the Coherent Matched-Filtering Algorithm}
The constraints we can place on MACHO abundance are a strong function of the maximum detectable flux ratio $R_f$ FRB brightness and the minimum delay $\tau_{min}$ resolvable by the telescope backend. These parameters in turn depends on the details of our correlation algorithm. In previous works, notably~\citet{sammons2020first}, the maximum detectable flux ratio is obtain using inspection of the light curves at high time resolution. In this work, we use a coherent matched filtering algorithm
analogous to those used in LIGO to search for lensed images. In this section we will relate the flux ratio $R_f$ to the brightness of the burst quantified by its SEFD and duration, using such a matched-filtering algorithm.

Our pipeline would be much simpler if we had an XF correlator, in which case we would collect actual raw voltage data instead of baseband. This ``XF pipeline'' can be thought of as an idealized version of our actual pipeline using baseband data (an FX correlator), and is a useful toy model. In this model, we'll neglect the effects of beamforming and coherent dedispersion, and assume that the burst is bright enough that our matched filter is optimal. Our data product is raw voltage data $v_i$, sampled every $1/(800\textrm{MHz})$. 

They can be modeled by
$$v_i = \sigma_n n_i + \sigma_s s_i\Pi_i  + \sigma_s \lambda \sqrt{\mu} s_{i-\hat{d}} \Pi_{i - \hat{d}}$$
where $n_i$ and $s_i$ are both gaussian random variables with zero mean and unit variance. $\sigma_n^2$ and $\sigma_s^2$ are positive quantities which parameterize the bandwidth-integrated system temperature and FRB temperature respectively. The gravitational lensing phenomenology is described by three variables: $\lambda = \pm 1$ (parity), $\sqrt{\mu}$ (magnification ratio), and $\hat d$, the true delay (in contrast to $d$, which is the trial delay over which we search). Finally we define $\Pi_i$, the pulse profile, which is sufficiently compact such that for all trial delays $d \geq d'$, $\Pi_{i \pm \hat{d}} \times \Pi_i = 0$ (i.e., it has zero overlap with itself). The pulse profile makes the voltage $v_i$ nonstationary, and introduces non-stationarity into our autocorrelation function.
%

Let's calculate the matched-filtered correlation function, using the pulse profile as a matched filter. Letting $h_i = \Pi^2_i$, the correlation function is
\begin{align}
    G(d) & \equiv \sum_{i} (v_i h_i) v_{i - d} = \sum_{i,j} \delta(i-j = d) (v_i h_i) v_j \\
    \intertext{where I've inserted a Kronecker delta function $\delta$. If we expand $v_i v_j$, there is an autocorrelation term proportional to $n\times n$ autocorrelation term, 2 autocorrelation terms proportional to $s\times s$, and 2 $s\times s$ cross terms, which appear in the presence of a coherent echo. Let's write all these terms separately, in that order:}
    n\times n = \sigma_n^2 \sum_{i,j} &\delta(i - j = d)  h_i n_i n_j \\
    &= \sigma_n^2 \delta( d = 0 )\sum_{i} \Pi_i^2\\
    \intertext{substituting $h_i \to \Pi^2_i $}
    s\times s \supseteq \sigma_s^2            \sum_{i,j} &\delta(i - j = d)  \Pi^2_i \Pi_i  \Pi_j  s_i s_j \mathrm{ (big auto)}\\
    s\times s \supseteq \varepsilon^2 \sigma_s^2 \sum_{i,j} &\delta(i - j = d)  \Pi^2_i \Pi_{i - \hat{d}} \Pi_{j - \hat{d}} s_{i - \hat{d}} s_{j - \hat{d}} \mathrm{ (small auto)} \\
    s\times s \supseteq \varepsilon \sigma_s^2   \sum_{i,j} &\delta(i - j = d)  \Pi^2_i \Pi_{i - \hat{d}} \Pi_j s_{i - \hat{d}} s_j \mathrm{ (anticross)}\\
    s\times s \supseteq \varepsilon \sigma_s^2   \sum_{i,j} &\delta(i - j = d)  \Pi^2_i \Pi_i  \Pi_{j - \hat{d}} s_{i} s_{j - \hat{d}} \mathrm{ (cross)}
    \intertext{Evaluate the delta function, substituting $j = i - d$, and assuming that $d > d'$}
    s\times s \supseteq \sigma_s^2            \sum_{i} &  \Pi^2_i \Pi_i  \Pi_{i - d}  s_i s_{i - d} \mathrm{ (big auto)}\\
    s\times s \supseteq \varepsilon^2 \sigma_s^2 \sum_{i} &  \Pi^2_i \Pi_{i - \hat{d}} \Pi_{{i - d} - \hat{d}} s_{i - \hat{d}} s_{{i - d} - \hat{d}} \mathrm{ (small auto)} \\
    s\times s \supseteq \varepsilon \sigma_s^2   \sum_{i} &  \Pi^2_i \Pi_{i - \hat{d}} \Pi_{i - d} s_{i - \hat{d}} s_{i - d} \mathrm{ (anticross)}\\
    s\times s \supseteq \varepsilon \sigma_s^2   \sum_{i} &  \Pi^2_i \Pi_i  \Pi_{{i - d} - \hat{d}} s_{i} s_{{i - d} - \hat{d}} \mathrm{ (cross)}
    \intertext{Take the expectation value over voltage realizations using $\langle s_m s_n \rangle = \delta(m = n)$}
    s\times s \supseteq \sigma_s^2            \sum_{i} &  \Pi^2_i \Pi_i  \Pi_{i - d}  \delta({d = 0}) \mathrm{ (big auto)}\\
    s\times s \supseteq \varepsilon^2 \sigma_s^2 \sum_{i} &  \Pi^2_i \Pi_{i - \hat{d}} \Pi_{{i - d} - \hat{d}}  \delta({d = 0}) \mathrm{ (small auto)} \\
    s\times s \supseteq \varepsilon \sigma_s^2   \sum_{i} &  \Pi^2_i \Pi_{i - \hat{d}} \Pi_{i - d}  \delta({d = \hat{d}}) \mathrm{ (anticross)}\\
    s\times s \supseteq \varepsilon \sigma_s^2   \sum_{i} &  \Pi^2_i \Pi_i  \Pi_{{i - d} - \hat{d}}  \delta({d = -\hat{d}}) \mathrm{ (cross)} \\
    \intertext{Now, pulling out the delta functions which don't depend on $i$, the final expectation for the correlation function is the sum of the following terms.}
    n\times n \supseteq \sigma_n^2 \delta({d = 0}) \sum_{i} & \Pi^2_i\mathrm{ (big noise)}\\
    s\times s \supseteq \sigma_s^2 \delta({d = 0})           \sum_{i} &  \Pi^2_i \Pi_i  \Pi_{i}   \mathrm{ (big auto)}\\
    s\times s \supseteq \varepsilon^2 \sigma_s^2 \delta({d = 0}) \sum_{i} & \Pi^2_i \Pi_{i - \hat{d}} \Pi_{i - \hat{d}}   \mathrm{ (small auto)} \\
    s\times s \supseteq \varepsilon \sigma_s^2 \delta({d = \hat{d}})  \sum_{i} &  \Pi^2_i \Pi_{i - \hat{d}} \Pi_{i - \hat{d}}   \mathrm{ (anticross)}\\
    s\times s \supseteq \varepsilon \sigma_s^2 \delta({d = -\hat{d}}) \sum_{i} &  \Pi^2_i \Pi_i  \Pi_{i}   \mathrm{ (cross)}\label{eq:signal}
\end{align}

Of these five terms, there are the three superimposed contributions at lag zero. One is due to the system background which is always present. We always see ``big auto'' and ``small auto'' and ``cross''. However, if the true lens delay $\hat{d}$ is large enough, $\Pi^2_i \Pi^2_{i - \hat{d}} = 0$ and we will not see the ``anticross'' peak at all. We are interested in the size of the signal: this is going to be the ``cross'' term.

The autocorrelation function separates different physical effects into different lag scales. At the shortest lag scales, $\tau < 2.56\mu s$, the analog bandpass filter and channel mask smear out peaks in $G(d)$. Optical bouncing of radio waves in the telescope structure and the analog chain on timescales similar to the light-travel time of the telescope  ($300$ ns) also affect this.
Next, at integer multiples of $2.56\mu$s, the PFB introduces temporal leakage artifacts as a side effect of suppressing frequency domain leakage. Next, because of the matched filtering, the ACF has different phenomenology for delays shorter than the duration $d'$ of the matched filter, which can be up to $3$ milliseconds. At lags greater than 3 milliseconds there is no physical effect which changes the phenonenology of the autocorrelation function. 

\subsection{Variance}
In addition to calculating the expectation value $\langle G(d) \rangle$ of this estimator, we can also calculate its variance. 
\begin{align}
    \langle G^2(d) \rangle &= \sum_{i,j,i',j'} \delta(i-j = d) \delta(i'-j' = d)\langle (v_{i} h_{i}) v_{j} (v_{i'} h_{i'}) v_{j'}\rangle \\ 
    \intertext{The product $\langle  v_{i} v_{j} v_{i'} v_{j'}  \rangle$ can be expanded with Wick's theorem}
    =&\sum_{i,j,i',j'} \delta(i-j = d) \delta(i'-j' = d) \langle v_i v_j    \rangle \langle v_{i'} v_{j'} \rangle h_{i} h_{i'} \\
    +&\sum_{i,j,i',j'} \delta(i-j = d) \delta(i'-j' = d) \langle v_i v_{i'} \rangle \langle v_j v_{j'} \rangle h_{i} h_{i'} \\
    +&\sum_{i,j,i',j'} \delta(i-j = d) \delta(i'-j' = d) \langle v_i v_{j'} \rangle \langle v_{i'} v_j \rangle h_{i} h_{i'} \\
    \intertext{Each of these expectation values is different from $\langle G(d) \rangle$ we calculated earlier since there's no matched filter in each expectation value. If we only keep the zero-lag contributions to $\langle v_i v_j \rangle$ and ignore the lensing signal's contribution to the variance we get}
    \langle v_i v_j \rangle &\approx \delta(i = j)(\sigma_n^2 + \sigma_s^2 \Pi_i \Pi_j)
    \intertext{Plug this in everywhere the average appears.}
    =& \langle G(d) \rangle^2 \\
    +&\sum_{i,j,i',j'} \delta(i-j = d) \delta(i'-j' = d)  \delta(i = i')(\sigma_n^2 + \sigma_s^2 \Pi_i \Pi_{i'})  \delta(j = j')(\sigma_n^2 + \sigma_s^2 \Pi_j \Pi_{j'}) h_{i} h_{i'}\label{eq:var1_4} \\
    +&\sum_{i,j,i',j'} \delta(i-j = d) \delta(i'-j' = d)  \delta(i = j')(\sigma_n^2 + \sigma_s^2 \Pi_i \Pi_{j'})  \delta(i' = j)(\sigma_n^2 + \sigma_s^2 \Pi_{i'} \Pi_j) \rangle h_{i} h_{i'}\label{eq:var2_4} \\
    \intertext{We are summing over 4 variables, but the terms only contribute when all delta functions are nonzero. We can kill two delta functions, kill the sums over primed indices, and algebraically replace the indices of Eq.~\ref{eq:var1_4}.}
    =&\sum_{i,j} \delta(i-j = d) (\sigma_n^2 + \sigma_s^2 \Pi^2_i) (\sigma_n^2 + \sigma_s^2 \Pi^2_j) h^2_{i}\\
    =&\sum_{i,j} \delta(i-j = d) (\sigma_n^4 + \sigma_s^2 \sigma_n^2 \Pi^2_i + \sigma_s^2 \sigma_n^2 \Pi^2_j + \sigma_s^4 \Pi^2_i \Pi^2_j) h^2_{i} \label{eq:var1}\\
    \intertext{In Eq.~\ref{eq:var2_4}, we replace all primed and unprimed $j$'s with their corresponding $i$'s and kill the sum over $j,j'$.}
    &\sum_{i,j,i',j'} \delta(i-j = d) \delta(i'-j' = d)  \delta(i = j')(\sigma_n^2 + \sigma_s^2 \Pi_i \Pi_{j'})  \delta(i' = j)(\sigma_n^2 + \sigma_s^2 \Pi_{i'} \Pi_j)  h_{i} h_{i'} \\
    =&\sum_{i, i'} \delta(i = i')\delta(d = 0)(\sigma_n^2 + \sigma_s^2 \Pi_i^2  )  (\sigma_n^2 + \sigma_s^2 \Pi^2_{i'} )  h^2_{i}  \\
    =&\sum_{i, i'} \delta(i = i') \delta(d = 0) (\sigma_n^4 + 2 \sigma_n^2 \sigma_s^2 \Pi_i^2 + \sigma_s^4 \Pi_i^4) h^2_{i} \label{eq:var2}
\end{align}
Combining Eq.~\ref{eq:var1},\ref{eq:var2}, the variance is $\langle G^2(d) \rangle - \langle G(d) \rangle^2$
\begin{align}
    =&\sum_{i,j} \delta(i-j = d) (\sigma_n^4 + \sigma_s^2 \sigma_n^2 \Pi^2_i + \sigma_s^2 \sigma_n^2 \Pi^2_j + \sigma_s^4 \Pi^2_i \Pi^2_j) h^2_{i}\\
    +&\sum_{i, i'} \delta(i = i') \delta(d = 0) (\sigma_n^4 + 2 \sigma_n^2 \sigma_s^2 \Pi_i^2 + \sigma_s^4 \Pi_i^4) h^2_{i} \\
    \intertext{Carry out the sum over $j$ and $i'$ in the first and second term respectively to kill the delta functions}
    =&\sum_{i} (\sigma_n^4 + \sigma_s^2 \sigma_n^2 \Pi^2_i + \sigma_s^2 \sigma_n^2 \Pi^2_{i-d} + \sigma_s^4 \Pi^2_i \Pi^2_{i-d}) h^2_{i}\\
    +&\sum_{i} \delta(d = 0) (\sigma_n^4 + 2 \sigma_n^2 \sigma_s^2 \Pi_i^2 + \sigma_s^4 \Pi_i^4) h^2_{i}
    \intertext{Replace $h^2$ with $\Pi^4$:}
    =&\sum_{i} \sigma_n^4 \Pi_{i}^4 + \sigma_s^2 \sigma_n^2 \Pi^2_i \Pi_{i}^4 + \sigma_s^2 \sigma_n^2 \Pi^2_{i-d} \Pi_{i}^4 + \sigma_s^4 \Pi^2_i \Pi^2_{i-d}h^2_{i} \label{eq:noise}\\
    +&\sum_{i} \delta(d = 0) \sigma_n^4\Pi_i^4 + 2 \sigma_n^2 \sigma_s^2 \Pi_i^2\Pi_i^4 + \sigma_s^4 \Pi_i^4\Pi_i^4
\end{align}

\subsection{Excursion Sets}
At the end of the correlation pipeline, we whiten the data by 1) dividing by the intensity autocorrelation, which measures the variance of the voltage autocorrelation as a function of lag, which has been normalized to 1 at zero lag. 2) Then, we normalize by the median absolute deviation in each (log-spaced) lag bin. The resulting statistic has unit variance and zero mean: it is a z-score, and a positive detection would show up as a large positive or negative fluctuation from the mean. To
quantify the size of the fluctuation, we calculate the z score from the above calculation by dividing Eq.~\ref{eq:signal} by Eq.~\ref{eq:noise}.

\begin{figure}
    \begin{center}
    \includegraphics[width = 0.5\textwidth]{./xf.png}
    \end{center}
    \label{fig:boxcar}
    \caption{A toy model where the FRB is Gaussian white noise modulated by a boxcar with $\varepsilon = 1$ (unrealistic), and $\sigma_n^2 = 40$ (realistic), $\sigma_s^2 = 2$ (realistic), and where the lensing delay exceeds the boxcar width (realistic). We have ignored the effects of beamforming, dedispersion, etc. on the voltage data. In reality there are $O(1)$ losses due to correlator segmentation, the PFB, beamforming, masked RFI channels, etc. which are difficult to
    characterize, so this is the most optimistic case.}
\end{figure}

\begin{align}
    \text{Signal} = \varepsilon \sigma_s^2 \delta({d = -\hat{d}}) & \sum_{i}  \Pi^2_i \Pi_i  \Pi_{i} \\ 
    \text{Noise}^2=&\sum_{i} \sigma_n^4 \Pi_{i}^4 + \sigma_s^2 \sigma_n^2 \Pi^2_i \Pi_{i}^4 + \sigma_s^2 \sigma_n^2 \Pi^2_{i-d} \Pi_{i}^4 + \sigma_s^4 \Pi^2_i \Pi^2_{i-d}\Pi_{i}^4 \\
    + &\sum_{i} \delta(d = 0) \sigma_n^4\Pi_i^4 + 2 \sigma_n^2 \sigma_s^2 \Pi_i^2\Pi_i^4 + \sigma_s^4 \Pi_i^4\Pi_i^4
    \intertext{To evaluate the sensitivity of our estimator quantified by the mean divided by the standard deviation (i.e., the Z-score), we need to plug in some expressions for $\Pi_i$. If we let
    the matched filter be a boxcar function centered at some $M_0$ with width $NM'$, as shown in Fig.~\ref{fig:boxcar},}
    \Pi_i^2 &= \begin{cases} 1 & |i - NM_0| < NM'/2 \\ 0 & \text{otherwise} \end{cases} \\
    \intertext{The moments of the matched filter become}
    \sum_{i} \Pi_i^{n} = \sum_{i} \Pi_{i-d}^n &= NM' \qquad \sum_{i} \Pi_i^n \Pi_{i-d}^{n'} = 0
    \intertext{The signal to noise at the lag $d = -\hat{d}$ is}
        \text{Signal}^2 &= (\varepsilon \sigma_s^2 (NM'))^2 \\
        \text{Noise}^2 &= (\sigma_n^4 (NM') + \sigma_s^2 \sigma_n^2 (NM') \\
        Z &= \dfrac{\varepsilon \sigma_s^2 (NM')}{\sqrt{(NM')(\sigma_n^4 + \sigma_s^2 \sigma_n^2)}} = \dfrac{\varepsilon \sigma_s^2 \sqrt{N M'}}{\sqrt{\sigma_n^2 + \sigma_s^2} \sqrt{\sigma_n^2}} \label{eq:low_snr}
    \intertext{I tried to numerically verify Eq.~\ref{eq:low_snr}. It works, but only in the low-SNR limit ($\sigma_s^2 / \sigma_n^2 << 1$): it underestimates the increase in the variance due to a bright burst. The SNR formula that worked was}
        Z &= \dfrac{\varepsilon \sigma_s^2 \sqrt{N M'}}{\sqrt{\sigma_n^2 + \sigma_s^2} \sqrt{\sigma_n^2 + \varepsilon^2 \sigma_s^2}} \label{eq:high_snr}
        \intertext{In our search pipeline we normalize $G(d)$ into SNR units empirically: first within each lag and then within each lag bin. Due to the look-elsewhere effect the largest excursion is typically of order $Z = 6$; this sets our noise floor to $Z > 6$. To translate this into magnification units we solve for $\varepsilon^2$ obtaining}
    R_f = \varepsilon^2 &= \dfrac{Z^2}{NM'} \dfrac{F^{-2} + F}{1 - \frac{Z^2 (1 + F)}{NM'}}
        \intertext{where $F = \sigma_s^2 / \sigma_n^2$.}
    \intertext{If we have a 2-Jansky FRB with a duration of $M'$ frames, and the system-equivalent flux density (SEFD) is 40 Jy, then $F =\sigma_s^2 / \sigma_n^2 = 2/40$. For a typical FRB (1.25 millisecond duration), the product $N M' \sim 10^6$, since CHIME samples voltages at 800 MHz. The above formula gives}
    R_f &\gtrsim 0.0144 \leftrightarrow 1/R_f = 69 \\
    \intertext{
    a comparable constraint to the two bright bursts that are used in the ASKAP analysis.
    }
\end{align}

